Removing Spurious Features can Hurt Accuracy and Affect Groups Disproportionately

The presence of spurious features interferes with the goal of obtaining robust models that perform well across many groups within the population. A natural remedy is to remove spurious features from the model. However, in this work we show that removal of spurious features can decrease accuracy due to the inductive biases of overparameterized models. We completely characterize how the removal of spurious features affects accuracy across different groups (more generally, test distributions) in noiseless overparameterized linear regression. In addition, we show that removal of spurious feature can decrease the accuracy even in balanced datasets -- each target co-occurs equally with each spurious feature; and it can inadvertently make the model more susceptible to other spurious features. Finally, we show that robust self-training can remove spurious features without affecting the overall accuracy. Experiments on the Toxic-Comment-Detectoin and CelebA datasets show that our results hold in non-linear models.

==> Makefile <==
TEXS=main.tex
ALLTEXS=$(shell ls *.tex)
ALLBIBS=$(shell ls *.bib)
PDFS=$(TEXS:.tex=.pdf)

default:
	pdflatex main
	bibtex main
	#latexmk -pdf main

jacob:
	latexmk -pdf main

all: $(PDFS)

clean:
	-rm *~ $(PDFS) *.aux *.bbl *.blg *.log *.out

%.pdf: $(ALLTEXS) $(ALLBIBS)
	pdflatex $(@:.pdf=.tex)
	bibtex $(@:.pdf=)
	pdflatex $(@:.pdf=.tex)
	pdflatex $(@:.pdf=.tex)

refs:
	@if [ ! -d "refdb" ]; \
	  then \
	  git clone https://github.com/percyliang/refdb;\
	fi
	cd refdb; git pull

run:
	go main.pdf


==> bias_proof.tex <==
\begin{proof}
	Let $\Sigma_{-s}=X^\top X$ and $\Sigma_{+s}= [X,s]^\top [X,s]$.
	Let $b_1,\dots,b_k$ be the basis of $Null(\Sigma_{-s})$.
	
	We know $s$ is a linear combination of columns of $X$, therefore, $Xt=s$.
	We know if $u \in \nl (\Sigma_{-s}) \implies [u,0] \in \nl (\Sigma_{+s})$.
	
	Now we find basis of $\nl (\Sigma_{+s}) = \{ [b_1,0], \dots, [b_k,0], [f,1]\}$
	
	we have:
	\begin{align}
	X^\top X f = -X s \implies f = -X^\dagger s
	\end{align}
(note that this results in $s^\top Xf = s^\top XX^\dagger s = t X^\top XX^\dagger Xt = tX^\top X t = s^\top s$).

now we can project $\theta^\star$ on $[f,1]$ since we assumed the weight of $s$ is $0$ in $\theta^\star$, the projection is:
\begin{align}
\ell \eqdef \frac{s^\top X^{\dagger\top} \theta^\star}{1+s^\top (X^\top X)^\dagger s} X^\dagger s = \frac{s^\top (X^\top X)^\dagger y }{1+s^\top (X^\top X)^\dagger s} (X^\top X)^\dagger (Xs)
\end{align}
Now let $\pi = (X^\top X)^\dagger (X^\top X)$ we have:
\begin{align}
\E [\theta_{-s} - \theta^\star] =& (I - \pi)\theta^\star\\
\E [\theta_{+s} - \theta^\star] =& (I - \pi)(\theta^\star - \ell) + \ell = (I - \pi)\theta^\star +\pi \ell = (I-\pi)\theta^\star + \ell
\end{align}

For every $\Sigma_g$ we have:

\begin{align}
B_{-s}(\Sigma_g) =& \E [\theta_{-s} - \theta^\star]^\top \Sigma_g \E [\theta_{-s} - \theta^\star]\\
=&((I - \pi)\theta^\star)^\top \Sigma_g (I - \pi)\theta^\star\\
B_{+s}(\Sigma_g) =& \E [\theta_{+s} - \theta^\star]^\top \Sigma_g \E [\theta_{+s} - \theta^\star]\\
=&((I-\pi)\theta^\star + \ell)^\top \Sigma_g ((I-\pi)\theta^\star + \ell)
\end{align}
therefore, a group has higher bias by adding $s$ if 
 weonsidering the last compoennet of $\ell$ we have:
\begin{align}
\ell^\top \Sigma_g (\ell + 2 (I-\pi)\theta^\star) + 2((I-\pi)\theta^\star + \ell)X_g^\top s_g a + as_g^\top s_g a
\end{align}

\end{proof}
Can we think of $\ell$ as the best prediction of $\theta^\star$ only using $s$?



==> bias_proof_2.tex <==
Assumption $Xt^\star = s$.

Define $\Pi = X^\top (XX^\top)^{-1}X$.

\begin{align}
\theta^{+s} =& X^\top (XX^\top)^{-1} (y-sw)\\
 =& \Pi \theta^\star - w\Pi t^\star\\
%w=&\frac{s^\top (XX^\top)^{-1}y}{1+s^\top(XX^\top)^{-1}s} \\
w=& \frac{{t^\star}^\top \Pi \theta^\star}{1+{t^\star}^\top\Pi t^\star}
\end{align}

Computing error for a group with $X_g$ and $s_g$.

\begin{align}
B(\theta^{+s} - \theta^{-s}) =& \E [\theta^\star - \theta^{+s}]^\top\Sigma_g \E [\theta^\star - \theta^{+s}] + 2\E [\theta^\star - \theta^{+s}]^\top X_g^\top s_g w + w s_g^\top s_g w \\
&- \E [\theta^\star - \theta^{-s}]^\top\Sigma_g \E [\theta^\star - \theta^{-s}]\\
=& ((I-\Pi)\theta^\star + wt)^\top \Sigma_g ((I-\Pi)\theta^\star +wt)+ 2((I-\Pi)\theta^\star + wt)^\top X_g^\top s_g w + w s_g^\top s_g w \\ 
&- ((I-\Pi)\theta^\star)^\top \Sigma_g ((I-\Pi)\theta^\star)\\
=&wt^\top \Sigma_g tw  + 2{\theta^\star}^\top (I-\Pi)\Sigma_g tw  + 2((I-\Pi)\theta^\star + wt)^\top X_g^\top s_g w + w s_g^\top s_g w \\
=&w^2\|s_g -X_gt\|_2^2 + 2{\theta^\star}^\top (I-\Pi) \Sigma_g tw + 2{\theta^\star}(I-\Pi)X_g^\top s_g w\\
=&w^2\|s_g -X_gt\|_2^2 + 2w{\theta^\star}^\top (I-\Pi) X_g^\top (X_g t + s_g)
\end{align}


Assuming $w>0$ we have:
\begin{align}
w^2\|s_g -X_gt\|_2^2 + 2w{\theta^\star}^\top (I-\Pi) X_g^\top (X_g t + s_g) >0\\
w > \frac{{\theta^\star}^\top (I-\Pi) X_g^\top (X_g t + s_g)}{\|s_g -X_gt\|_2^2}
\end{align}

==> bias_proof_3.tex <==
\section{Over parametrized regime}

\subsection{Bias variance decomposition}

\subsection{the rest}



 
 This formulation look at the project of $\theta^\star$ on $t^\star$ on two different space:
 1) the column space of $X^\top X$ (let's call this $w$)
 2) the null space of $X^\top X$ and then rescaled/rotate with $\Sigma$ (let's call this $w'$).
 This formulation simply state that:
 \begin{align}
 \frac{w}{2} \le {w'}
 \end{align}
 in this case using $s$ helps and if the equation is the other way around using $s$ hurts the accuracy.
 



==> comparison_table.tex <==
\begin{table}
	\centering
	\begin{tabular}{llll} \toprule
		model & weight on $s$  & weight on $z$ &weight on $z$  \tiny (another formulation) \\ \midrule
		with $s$& $w$  &$\Pi \theta^\star - w\Pi t^\star$ &  $\theta^{+s}$ \\ 
		no $s$ & $0$ & $\Pi \theta^\star$ &$\theta^{+s} + w\Pi t^\star$\\ 
		no $s$ and self-train & $0$ & $\Pi \theta^\star + w(    \mathbb{I}-\Pi)t^\star$ & $\theta^{+s} + wt^\star$\\ \bottomrule
	\end{tabular}
	
		\centering
		\begin{tabular}{lll} \toprule
			model & loss &\\ \midrule
			with $s$&  $\E [(y - z\theta + wzt- ws)^2]$= &$\E (y-z\theta)^2] + w^2 \E [(s-zt)^2] - 2w \E[ (y -z\theta) (s-zt)]$\\ 
			no $s$ & $\E [(y - z\theta)^2]$ = & $\E (y-z\theta)^2]$  \\ 
			no $s$ and self-train &  $\E [(y - z\theta + wzt - wzt^\star)^2]$ =   & $\E (y-z\theta)^2] + w^2 \E [(zt^\star - zt)^2] - 2w \E[ (y -z\theta)(zt^\star - zt)]$ \\ \bottomrule
		\end{tabular}
		
%			\centering
%			\begin{tabular}{lll} \toprule
%				model & loss \tiny (another formulation) &\\ \midrule
%				with $s$&  $\E [(y - z\theta^{+s} - ws)^2]$= &$\E (y-z\theta^{+s})^2] + w^2 \E [s^\top s] - 2w \E[ (y -z\theta^{+s})^\top s]$\\ 
%				no $s$ & $\E [(y - z\theta^{+s} - wz\Pi t^\star)^2]$ = & $\E (y-z\theta^{+s})^2] + w^2 \E [{t^\star}^\top \Pi \Sigma \Pi t^\star] - 2w \E[ (y -z\theta^{+s})^\top z\Pi t^\star]$ \\ 
%				no $s$ and self-train &  $\E [(y - z\theta^{+s} - wzt^\star)^2]$ =   & $\E (y-z\theta^{+s})^2] + w^2 \E [{t^\star}^\top\Sigma t^\star] - 2w \E[ (y -z\theta^{+s})^\top zt^\star]$ \\ \bottomrule
%			\end{tabular}
\end{table}

==> connection_to_DRO.tex <==
\subsection{min-max (group DRO) does not help}
Here since everything is convex min-max is like re-weighting. 
For some fixed \tre{} group point according to $s$ and \tre{}, i.e., we have the following four groups:
\begin{itemize}[nosep]
	\item $g_{11}: s=1, y \ge \tre$
	\item $g_{10}: s=1, y < \tre$
	\item $g_{01}: s=0, y \ge \tre$
	\item $g_{00}: s=0, y < \tre$
\end{itemize}

According to \refprop{hurt}, under some condition then using $s$ might hurts some of these groups.
Even minimizing maximum loss fo these groups, still it is possible that group have lower loss when we do not use $s$ completely.

==> extra_figures.tex <==
\section{Extra figures}
\input{percentage_tabular}

==> groups_with_different_functions_on_s.tex <==
\section{Multiple Groups with different functions on the spurious feature}
So far, we assumed that the parameter to predict the spurious feature is the same for both groups. 
In this section, we assume the function for $y$ is the same for all groups (i.e, $y = \theta^\top z$), but different groups have different functions for the spurious features. 
For simplicity we assume we only have two groups (we can generalize the formulation to multiple groups, see \refsec{})
Let $\alpha_{i}$ be the coefficient for predicting $s$ for  of the $i^\text{th}$ group (i.e., $s = \alpha_g^\top z$).

Previously, we observed that the predictor use the following implicit bias: if $\theta$ and $\beta$ are correlated in $\Pi$ then they are correlated in $I-\Pi$ as well; and we observed that the average accuracy drop if the correlation between $\theta$ and $\beta$ are different in $\Pi$ and $I-\Pi$.

Now what happens if groups have different function for the spurious feature.
We first stat with a simple example to understand the implicit bias in this case.



\begin{example}
	 Let $Z = \begin{bmatrix}
	 1 & 0 \\
	 0 & 1
	 \end{bmatrix}$, let $y = \theta= [1,1]$, $\alpha_1=[2,2]$, and $\alpha_2 = [-1,-1]$, then we have $s = \hat \alpha = [2,-1]$.
	 In this case, $w=\frac{1}{6}$ and $\hat\theta = [1-2w, 1 + w]$.
	 As a result if in the test time we see $[1,0]$ from the second group (note that we only see $[1,0]$ from the first group in the training) then we predict $\hat y = 1-3w$ (instead of the true value $y=1$). 
	 Similarly, if we see $[0,1]$ from the first group in the test time (note that we only see $[0,1]$ from the second group in the training) then we predict $hy = 1 + 3w$ (instead of the true value $y=1$).
%	 let $\theta= [1,1,1,1]$, $\alpha_1=[2,2,2,2]$, and $\alpha_2 = [-1,-1,-1,-1]$, then we have $\hat \alpha = [2,2,-1,-1]$
\end{example}



Let $Z_1 \in \BR^{n\times d}$ be data points in group 1 and $Z_2 \in \BR^{n \times d}$ be data points in group 2.
We first compute estimated $\hat \beta$.

\begin{align}
min \quad&\|\hat \beta\|\\
s.t. \quad& Z_1 \hat \beta = Z_1 \beta_1\\
&Z_2 \hat \beta = Z_2 \beta_2
\end{align}

\citet{} shows how to compute the projection matrix for intersection of two subspaces.
In our case we are interested in projection of $\Pi_1$ and $\Pi_2$.
\begin{align}
\Pi_{1\cap 2} = 2\Pi_1 (\Pi_1 + \Pi_2)^\dagger \Pi_2
\end{align}

Using this equation and Schur compliment we can compute $\hat beta$ as follows:
\begin{align}
M &= Z_1^\top (Z_1 (I-\Pi_2)Z_1^\top)^{-1}Z_1\\
N &= Z_2^\top (Z_2 (I-\Pi_1)Z_2^\top)^{-1}Z_2\\
\hat \alpha &= (I-\Pi_2)M\alpha_1 + (I-\Pi_1)N\alpha_2
\end{align}

For simplicity let assume $\Pi_1$ and $\Pi_2$ are orthogonal (i.e., $\Pi_1\Pi_2=0$) then we have:


\begin{align}
\hat \theta = Z^\top (ZZ^\top)^{-1} (y-sw) = \Pi \theta -w \Pi_1\alpha_1 -w \Pi\alpha_2
\end{align}

Now we can compute the error for group 1 as follows:
\begin{align*}
\E \pb {\p {\theta^\top z - \hat{\theta}^\top z + w\hat\alpha z - w \alpha_1^\top z}^2}=&  \E \pb {\p {\theta^\top z - (\Pi \theta)^\top z + w\alpha_1^\top \Pi_1 z + w\alpha_2^\top\Pi_2 z - w \alpha_1^\top z}^2}\\
=&  \E \pb {\p {\theta^\top (I-\Pi) z - w\alpha_1^\top (I-\Pi_1) z + w\alpha_2^\top\Pi_2 z}^2}\\
=& \theta^\top (I-\Pi)\Sigma(I-\Pi)\theta \\
&+ w^2 \alpha_1^\top (I-\Pi) \Sigma (I-\Pi_1) \alpha_1 -2w \theta (I-\Pi) \Sigma (I-\Pi_1) \alpha_1\\
&+w^2 \alpha_2 \Pi_2 \Sigma \Pi_2 \alpha_2  - 2w^2\alpha_2^\top \Pi_2\Sigma (I-\Pi_1)\alpha_1 + 2w \alpha_2\Pi_2\Sigma (I-\Pi) \theta
\end{align*} 




==> omitted_bias.tex <==
\section{Omitted variable bias}
\fk{TODO}
We now look at a setup in which some of the features are missing, but we have access to infinite data.
Omitted variable bias has been studied in statistics and economics (e.g.,  \cite{clarke2005phantom})
Formally, let $X \in \BR^{n\times p}$ be the observed covariates, $Z \in \BR^{n\times q}$ be unobserved covariates and $y \in \BR^n$ be the response such that $y = X\beta + Z\delta + U$, where $U$ is mean zero condition on $X$ and $Z$. Estimating $\beta$ using least-squares estimator we have: 
\begin{align}
\E [\hat \beta] = \beta + \underbrace{(X^\top X)^{-1} \E [XZ \mid X] \delta}_{\text{bias}}
\end{align}

In this work we are interested in a general characterization of the groups which they loss will increase if in addition to $X$ we observe one column of $Z$ as well.


%\begin{corollary}
%Same as the previous paper:
%    \begin{align}
%    &\pr (z) =\pr [s=0] \pr[z\mid s=0] +\pr [s=1]\pr [z \mid s=1] \nonumber\\
%    &y = \beta z \nonumber\\
%    &x = z +u
%    \end{align}
%    Under some simplifying assumptions: everything is one-dimensional and slope does not change (should be fixed) the following holds:
%    
%    
%
%        \label{prop:hurt} Let $\mu = \E [z]$, $\mu_{s=0}=\E [z \mid s=0]$, and $\mu_{s=1}=\E [z \mid s=1]$.
%        Let $g$ be a subgroup of point with $s=s'$.
%        If $
%        |\E [z \mid g=1] - \mu| \le |\E [z \mid g=1] - \mu_{s=s'}|$, then $\E [\ell (h_{+s}) \mid g=1] \ge \E [\ell (h_{-s})\mid g=1]$.
%
%    
%    \begin{proof}
%        \begin{align*}\E [\ell (h_{+s}) \mid g=1] - \E [\ell (h_{-s})\mid g=1]=(\Lambda\beta) (\mu_{s=1} - \mu_{s=0}) (\mu_{s=1} + \mu_{s=0} -2\E [z \mid g=1])
%        \end{align*}
%    \end{proof}
%    \end{corollary}




\subsection{General characterization}
Let $x \in \BR^{p}$ denote the observed variables, 
let $s \in \BR$ be only available to $h_{+s}$,
and let $z \in \BR^{n\times q}$ be the unobserved variables. 
Let $y= \alpha^\top x + \beta s + \gamma^\top z$.
%(note that when $T$ is one dimensional and independent of $z$ and $x$ then we are in the common setup in which $y = \alpha^\top x + \beta^\top z + \epsilon$.).
We are interested in groups for them the $h_{-s}$ (although having less information) lead to higher accuracy than the $h_{+s}$.

\begin{proposition} WLOG, let $x=0, \E [s \mid x=0]=0$ and  $\E [z \mid x=0]=0$. Let $\lambda = \Sigma_{ss}^{-1}\Sigma_{sz}$, and WLOG assume $\lambda^\top \gamma + \beta >0$.
Fix a group $g$ and let $\lambda_g = \Sigma_{ss \mid g=1}^{-1}\Sigma_{sz\mid g=1}$, then $\E [\ell (h_{+s}) \mid g=1] \ge [\ell(h_{-s}) \mid g=1]$ iff $\gamma^\top (\lambda - 2\lambda_g) \ge \beta$.
	
\end{proposition}

\begin{proof}
	\begin{align}
	\E [\ell(h_{+s}) \mid g=1] - \E [\ell(h_{-s}) \mid g=1] =&
	\E [	(\gamma^\top z - \gamma^\top \lambda s)^2 - (\gamma^\top z + \beta s)^2 \mid g=1]\\
	=& \E [(\gamma^\top \lambda s)^2 - 2\gamma^\top zs\lambda^\top \gamma  - (\beta s)^2 - 2\gamma^\top zs \beta \mid g=1]\\
	=& \E [ ((\gamma^\top \lambda)^2 - \beta^2)s^2 - 2 \gamma^\top zs (\lambda^\top \gamma + \beta) \mid g=1]\\
		=& ((\gamma^\top \lambda)^2 - \beta^2) \E [s^2 \mid g=1] - 2 \gamma^\top \E [zs \mid g=1] (\lambda^\top \gamma + \beta) 
\end{align}
We are interested if the RHS is greater than zero. We assume $\lambda^\top \gamma + \beta >0$ (Other cases are solved similarly). and divide the RHS sides by it.
dividing RHS by $\E [s^2 \mid g=1]$ completes the proof.
\begin{align}
(\gamma^\top \lambda - \beta)  - 2 \gamma^\top \lambda_g \ge 0\\
\gamma^\top (\lambda - 2\lambda_g) \ge \beta
\end{align}
\end{proof}
	
This proposition states that in order for a group to prefer $h_{-s}$ over $h_{+s}$, $\gamma$ (the coefficient of unseen data) should be larger than $\beta$ (the coefficient of $s$), and the correlation in $g$ should be different from the correlation between $s$ and $z$ in the whole dataset.

\subsection{Simple Example}

Let $s \sim Bernouli (0.5)$ and $x \sim \sN(s,\sigma)$, $y=s + \gamma x$.
As before, let $\theta_{+s}$ be the linear estimator using $s$ and $\theta_{-s}$ be the one without $s$. We are interested in groups such that $\E [\ell(h_{+s}) \mid g=1] > \E [\ell(h_{-s}) \mid g=1]$.
$h_{-s}$ predict $1$ for all data points. $h_{+s}$ on the other hand predict differently for different $s$. $h_{+s}(s=0) = 0$ and $h_{+s}(s=1) = 2$.
Obviously, if we define $g$ to be all points with $s=0$ and $x>1.5$ or $s=1$ and $x < 1.5$ they have lower loss when $s$ is note used at all.

%Note that using $z_1$ causes lower loss for overall data points and for each group according to $z_1$.
%\begin{itemize}
%	\item $\E [\ell_2] \le \E [\ell_1]$
%	\item $\forall u: \quad \E [\ell_2 \mid z_1=u] \le \E [\ell_1 \mid z_1=u]$
%\end{itemize} 
%
%However, if we group points according to $z_1$ \emph {and $z_2$}, then there exists some groups which prefer the second predictor over the first one.

%\begin{table}\centering
%	\begin{tabular}{rrr}
%		&infinite data but missing information & all information but low training data\\ \midrule
%		linear regression &&\\ \midrule
%		logistic regression &&\\ \bottomrule
%	\end{tabular}
%	\caption{We are interested to study the effect of using a new feature on accuracy across group on these four setups.}
%\end{table}


==> percentage_tabular.tex <==

\begin{table}
	\centering
\scalebox{0.5}{
	\begin{tabular}[width=0.2\textwidth]{lccc} 	\toprule
		\bf adjective & \bf positive & \bf negative & \bf positive/negative ratio\\ \midrule
all &  13.56 & 86.44 & 0.16 \\
gay & 4.20 & 3.10 & 1.36 \\
homosexual & 0.75 & 0.95 & 0.79 \\
straight & 0.51 & 4.34 & 0.12 \\
male & 0.32 & 2.61 & 0.12 \\
female & 0.28 & 2.65 & 0.10 \\
black & 1.24 & 8.09 & 0.15 \\
white & 1.28 & 8.83 & 0.14 \\
european & 0.29 & 5.00 & 0.06 \\
american & 1.25 & 15.74 & 0.08 \\
indian & 0.39 & 4.84 & 0.08 \\
chinese & 0.40 & 4.24 & 0.10 \\
christian & 0.44 & 6.27 & 0.07 \\
muslim & 0.46 & 3.76 & 0.12 \\
jewish & 0.58 & 5.75 & 0.10 \\
old & 2.47 & 21.42 & 0.12 \\
young & 0.31 & 4.40 & 0.07 \\ 
blind & 0.32 & 1.84 & 0.17 \\
\bottomrule
	\end{tabular}}
\caption{\label{tab:identity_terms} The 17 adjectives that we use as identity terms (spurious features) along with the percentage of positive and negative comments containing the adjectives.}
\end{table}

==> prev_examples.tex <==




%\section{Over Parametrized regime}
%In this section, we study the effect of using a new feature for linear regression in over parametrized regime. 
%Let $X \in \BR^{n\times d}$ be the observed covariates and $y \in \BR^n$ be the response. We assume we are in over parametrized regime, $n < d$.
%Using least-norm estimate we have
%\begin{align}
%\label{eqn:nos}
%\theta^{-s} = \argmin \| \theta\|_2^2\\
%s.t. \quad X\theta =y.
%\end{align}
%\\\
%With abuse of notation, let $s \in \BR^n$ denote the values of feature $s$ for the $n$ data points. Using this new feature our estimate is: 
%\begin{align}
%\label{eqn:withs}
%\theta^{+s} = \argmin \| \theta\|_2^2 + w^2\\
%s.t. \quad X\theta + sw =y,
%\end{align}
%where the variable $w$ denote the weight associate with the feature $s$.
%
%For the first scenario \refeqn{nos} we have: 
%\begin{align}
%\theta^{-s} = X^\dagger X\theta^\star
%\end{align}
%In the second scenario, when we use feature $s$ we have:
%\begin{align}
%\label{eqn:w_sol}
%\theta^{+s} &= X^\dagger(X\theta^\star-sw)
%\end{align}
%
%Taking derivative and minimizing the L2-norm we have:
%\begin{align}
%(X^\dagger X\theta^\star-X^\dagger sw)^\top(X^\dagger X\theta^\star-X^\dagger sw) + w^2\\
%-2ws^\top X^{\dagger\top}X^\dagger X\theta^\star + ws^\top X^{\dagger\top}X^\dagger sw + w^2\\
%-2s^\top X^{\dagger\top}X^\dagger X\theta^\star + 2ws^\top X^{\dagger\top}X^\dagger s + 2w\\
%w = \frac{s^\top (X^\top X)^\dagger y}{1 + s^\top (X^\top X)^\dagger s} = \frac{s^\top X^{\dagger \top} \theta^\star}{1 + s^\top (X^\top X)^\dagger s}\\\\
%\theta^{+s} = X^\dagger X\theta^\star - \frac{s^\top X^{\dagger \top}\theta^\star}{1 + s^\top (X^\top X)^\dagger s}X^\dagger s
%\end{align} 
%
%\begin{align}
%\theta^{+s} &= X^\dagger(X\theta^\star-sw)\\
%w &= \frac{y^\top (X^\top X)^\dagger s}{1+ s^\top (X^\top X)^\dagger s}
%\end{align}
%
%Intuitively, if $s$ is correlated with $y$ then $w$ is bigger and $\theta^{+s}$ is smaller than $\theta^{-s}$.
%
%
\subsection{Examples}

Let $n=d=3$ and the observed examples form an identity matrix, $Z = I$, thus $\Pi = I$. 
Let $s_1 = [0,1,1]^\top$, thus $\beta_1 = [0,1,1]^\top$ and similarly, let $s_2 = \beta_2 = [1,1,0]^\top$. Let the prediction target $y = \theta = [1,1,1]^\top$.



\paragraph{Example 1.}
Let $n=d$, and $X$ be the identity matrix. 
Let $\theta^\star = \bold 1$, and $y = X\theta^\star$.
Let feature $s$ be the spurious feature which is $1$ with probability $p$, and $0$ with probability $1-p$.
We are interested in the error of $\theta^{+s}$ in the population.
Note that, in this example, the only random vector is $s$, and the rest of the parameters are fixed, all the expectations are regarding the values of $s$.
Since $X=I$ then $(X^\top X)^\dagger=I$.
Let $u \sim \text{binomial}(n,p)$ be random variable denotes number of points with feature $s=1$, we have:
\begin{align}
&\E [w] = \E [\frac{u}{1+u}] = 1-\E [\frac{1}{1+u}] = 1-\frac{1-(1-p)^{n+1}}{(n+1)p}\\
&\E [\theta^{+s}_i]= 1- \frac{\E [uw]}{n} = 1-p + \frac{\E [w]}{n}
%&\E [({\theta^{+s}_i})^2]
\end{align}





\begin{figure}
	\centering
	\begin{subfigure}[b]{0.45\textwidth}\centering
		\includegraphics[width=0.35\textheight]{images/diff_n.png}
		\caption{\label{fig:diff_n}$\E [\ell]$ and $\E [\ell \mid s=0]$ and $\E [\ell \mid s=1]$, for $p=0.9$ and different values of $n$.}
	\end{subfigure}\hfill
	\begin{subfigure}[b]{0.45\textwidth}\centering
		\includegraphics[width=0.35\textheight]{images/diff_p.png}
		\caption{\label{fig:diff_p}$\E [\ell]$ and $\E [\ell \mid s=0]$ and $\E [\ell \mid s=1]$, for $n=20$ and different values of $p$.}
	\end{subfigure}
	
\end{figure}

As $n$ (which we assumed is also equal to $d$ as the number of features) increases, the model rely more on $s$ (i.e., $\E [w]$ increases and $\E [\theta^{+s}_i]$ decreases).
Due to the spurious correlation if we group points according to the feature $s$ (i.e., $\E [\ell \mid s=1]$ and $\E [\ell \mid s=0]$) they incur different losses. 
As $n$ (\reffig{diff_n} and \ref{fig:diff_p}).

As a final note, in this example, we assumed $s$ is correlated with $y$ for all the data points.
However, if $s$ is only correlated with $y$ for a particular group, then using $s$ will adversely effect individuals on that groups that do not obey the correlation.
%For example, We can have $s$ to be correlated with $y$ only for data points that one of the first $d/2$ features are $1$.
%Then, in this example, the loss for different groups are as follows:
%\begin{align}
%\E [\ell \mid s=1, \theta_{1:d}> 1] = \\
%\E [\ell \mid s=1, \theta_{1:d}< 1] = \\
%\E [\ell \mid s=0, \theta_{1:d}> 1] = \\
%\E [\ell \mid s=0, \theta_{1:d} < 1] = 
%\end{align}


\paragraph{Example 2.}

In the previous example, it is clear that removing feature $s$  improves the error for all groups. 
We now consider a more complicated setup in which removing $s$ increases the average error overall (as well as some groups). 
Like before, assume $X=I$. In this example, we have two extra features $s$ as before, and $t$ which is $1$ with probability of $0.5$ for all data points. 
Let $w_s$ denote the weight for the feature $s$, and $w_t$ denote the weight for the feature $t$ we have: 

%\begin{align}
%w_s &= \frac{(y-w_tt)^\top (X^\top X)^\dagger s}{1+s^\top (X^\top X)^\dagger s}\\
%w_t &= \frac{(y-w_ss)^\top (X^\top X)^\dagger t}{1+t^\top (X^\top X)^\dagger t}\\
%\theta &= 1 - sw_s - tw_t\\
%\end{align}
%
%\fk{TODO: compute the expectation over $s$ and $u$}

\reffig{exam_2} shows when we use $s$, the error of the model is only high for the group with $s=0$; however, when we remove $s$ in training (the model increase $w_t$) which leads to an increase for the average error as well as the group with $s=1$.



\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{images/example_2.png}
	\caption{\label{fig:exam_2}Without using the feature $s$ the model start using the feature $t$ which lead to higher error in average (but lower error for group with $s=0$).}
\end{figure}

%\subsection{General characteristics}
%Let $X_{+s}= [X,s]$ and $X_{-s} = [X, 0]$. define $\hat \Sigma_{+s} = X_{+s}^\top X_{+s}$ and $\hat \Sigma_{-s} = X_{-s}^\top X_{-s}$. 
%
%As we know, for a general least norm estimate we have: $\E [\theta - \theta^\star] = (I - (X^\top X)^\dagger (X^\top X))\theta^\star$ which is the projection of $\theta^\star$ on the null space of $X^\top X$).
%
%\fk{this is confusing but I can make it clear with a picture}
%We assumed the dimension of $s$ in $\theta^\star$ is zero so WLOG we can assume $\var (s)$ in $\hat \Sigma_{-s}$ is $1$ instead of $0$, so we can be sure the dimension of $s$ in the bias is always zero for any estimator.
%
%Therefore, we have $Null(\Sigma_{-s}) \subseteq Null(\Sigma_{+s})$ (therefore, we always have a better parameter estimator). However the error can increase for some groups (even in average).
%Let $\Sigma_g$ be the covariance matrix for a group $g$, Using Michael's paper terminology a group error will increase by removing $s$ if 
%\begin{align}
%v^\top\Sigma_g v < -2w^\top\Sigma_g v
%\end{align}
%
%
%%where $v = \Pi^\upvdash_{+s} \Pi_{-s}\theta^\star$ and $w=\Pi_{-s}^\upvdash\theta^\star$.
%
%
%This general result is not intuitive! we can actually find out more intuitive result using \refeqn{w_sol}.
%
%\paragraph{claim:} I believe we can come up with a result which shows a group will have lower loss without using $s$ if predicting $y$ only using $s$ will have high error on that group. 



%\paragraph{Example 3.} Let $y = z_1$. Assume that we only have one example ($z_1=1, y=1$)! Consider the following two predictors:
%\begin{itemize}
%%    \item No feature is available, $\hat{y_1}$ is simply average for all data points $\hat y_1 = \E [z_1] + \E [z_2]$.
%    \item $z_1$ is available but $z_2$ is not available $\hat y_2 = z_1$ (i.e., $\beta_1 = 1$)
%    \item $z_1$ and $z_2$ are available then we have $\hat \beta_1 = \frac{1}{1+z_2^2}, \beta_2= \frac{z_2}{1+z_2^2}$.
%\end{itemize}
%Is there any groups defined on $z_1$ which prefer the second predictor over the first one? (this is become more interesting when we have two features instead of only one.)
%
%Intuition: Groups for which 
%$\beta_3$ is meaningful prefer the second predictor while other groups prefer the first predictor.


==> questoin_and_answer.tex <==
\paragraph{Question.} 
Assume we have $n$ data points in $d$ dimensions.
Let $s$ be a new feature. Let $h_{+s}$ be a predictor which uses $s$, and let $h_{-s}$ be a predictor that does not use $s$. 
For which groups using $s$ leads to higher loss (i.e., $\E[\ell (h_{+s}) \mid g=1] > \E [\ell (h_{-s}) \mid g=1]$)?


\paragraph{Answer.} In this work, we study the effect of using a new feature for linear regression in two cases: 1) over parametrized regime and 2) missing information regime.
For the first case, we study a setup that all the features exist (no missing information) and show even when $s$ has ``spurious'' correlation with $y$, removing $s$ can increase the overall error.
For the second case, we study infinite data setup (no over parametrization) and show that even when $s$ is a true feature for $y$, using $s$ can lead to higher error for some groups.
\section{General Setup}
We have a set of features $x \in \BR^{d_x}$, we divide $x$ into two sets $z\in \BR^{d_z}$ and $s\in \BR^{d_s}$. 

We call $s$ is a spurious feature if:
\begin{align}
\pr [y \mid z,s] = \pr [y \mid z]
\end{align} 


We call $s$ is a strict spurious feature if:
\begin{align}
\pr [y \mid s] = \pr [y]
\end{align}

Let $\sP_z$ denote the underlying distribution for the core features $z \sim \sP_z$. 
Let target be a function of the core features $y = f(z,u)$, and the spurious features can also be a function of the core features $s = g(z,v)$ where $u$ and $v$ denote the source of randomness. 


\paragraph{Main questions:} Under what conditions omitting $s$ helps/hurts accuracy? 

==> setup_picture.tex <==
%\begin{SCfigure}
%\begin{tabular}{c}{\begin{align*} 
%\begin{bmatrix}[ccc|c]
%z_{11} & \dots & z_{1d} & s_1\\
%\vdots & \ddots & \vdots & \vdots\\
%z_{n1} & \dots & z_{nd} & s_n
%\end{bmatrix} \times
%\begin{bmatrix}
%\hat \theta_{1}\\
%\vdots\\
%\hat{\theta}_{d}\\
%w
%\end{bmatrix} = 
%\begin{bmatrix}
%y_{1}\\
%\vdots\\
%y_{n}
%\end{bmatrix} 
%\end{align*}}
%\end{tabular}
%\caption{feri}
%\end{SCfigure}


\begin{figure}
	\begin{minipage}[c]{0.6\textwidth}

{\begin{align*} 
	\begin{bmatrix}%[ccc|ccc]
	z_{11} & \dots & z_{1d} & s_{11} & \dots & s_{1k}\\
	\vdots & \ddots & \vdots & \vdots &\ddots & \vdots\\
	z_{n1} & \dots & z_{nd} & s_{n1} & \dots & s_{nk}
	\end{bmatrix} \times
	\begin{bmatrix}
	\hat \theta_{1}\\
	\vdots\\
	\hat{\theta}_{d}\\
	w_1\\
	\vdots\\
	w_k
	\end{bmatrix} = 
	\begin{bmatrix}
	y_{1}\\
	\vdots\\
	y_{n}
	\end{bmatrix} 
	\end{align*}}
	\end{minipage}\hfill
	\begin{minipage}[c]{0.35\textwidth}
		\caption{
the setup considered in this paper, $z_1,\dots,z_d$ are the core features, $s_1,\dots,s_k$ are the spurious features. We assume $y={\theta^\star}^\top z$ and $s_i = {\beta^\star_i}^\top z$.
		} \label{fig:03-03}
	\end{minipage}
\end{figure}
